Pouring by Feel: An Analysis of Tactile and Proprioceptive Sensing for Accurate Pouring

As service robots begin to be deployed to assist humans, it is important for them to be able to perform a skill as ubiquitous as pouring. Specifically, we focus on the task of pouring an exact amount of water without any environmental instrumentation, that is, using only the robot's own sensors to perform this task in a general way robustly. In our approach we use a simple PID controller which uses the measured change in weight of the held container to supervise the pour. Unlike previous methods which use specialized force-torque sensors at the robot wrist, we use our robot joint torque sensors and investigate the added benefit of tactile sensors at the fingertips. We train three estimators from data which regress the poured weight out of the source container and show that we can accurately pour within 10 ml of the target on average while being robust enough to pour at novel locations and with different grasps on the source container.

==> evaluation.tex <==
\section{Evaluation}

Our objective is to replace the force sensor used at training time with a regressor which can continuously output the current poured weight out of the source container. In the previous section we described three different estimators to be trained using either only tactile, only end effector forces or both modalities. We also propose the use of an analytical formulation where we take the $z$ component of the computed forces at the end effector in robot coordinates as a baseline comparison. 

Our first evaluation of these methods will consist in comparing their individual predictions against ground truth on our collected test set, composed of 20 randomly selected trials. 

We evaluate these methods by deploying them in real-time on our robot arm and performing a set of representative pouring trials, both within and outside the training data distribution. Table \ref{tab: eval_trials} describes 12 instances of pouring trials with various parameters that sweep through different pouring speeds, liquid volume at the source container and target volume to achieve on the receiving container.




\begin{table}[]
\centering
\caption{Evaluation trials parameters}
\label{tab: eval_trials}
\begin{tabular}{lccc}
Trial \# & \begin{tabular}[c]{@{}c@{}}Pour speed \\ {[}ml/s{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Source volume\\ {[}ml{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Target volume\\ {[}ml{]}\end{tabular} \\ \hline
1  & 15  & 220  & 120 \\
2  & 45 & 220 & 120 \\
3  & 80 & 220 & 120 \\
4  & 15 & 220 & 180 \\
5  & 45 & 220 & 180 \\
6  & 80 & 220 & 180 \\
7  & 15 & 320 & 150 \\
8  & 45 & 320 & 150 \\
9  & 80 & 320 & 150 \\
10 & 15 & 320 & 260 \\
11 & 45 & 320 & 260 \\
12 & 80 & 320 & 260                                    
\end{tabular}
\end{table}
